Enhancing Security Patch Identification by Capturing Structures in Commits

With the rapid increasing number of open source software (OSS), the majority of the software vulnerabilities in the open source components are fixed silently, which leads to the deployed software that integrated them being unable to get a timely update. Hence, it is critical to design a security patch identification system to ensure the security of the utilized software. However, most of the existing works for security patch identification just consider the changed code and the commit message of a commit as a flat sequence of tokens with simple neural networks to learn its semantics, while the structure information is ignored. To address these limitations, in this paper, we propose our well-designed approach E-SPI, which extracts the structure information hidden in a commit for effective identification. Specifically, it consists of the code change encoder to extract the syntactic of the changed code with the BiLSTM to learn the code representation and the message encoder to construct the dependency graph for the commit message with the graph neural network (GNN) to learn the message representation. We further enhance the code change encoder by embedding contextual information related to the changed code. To demonstrate the effectiveness of our approach, we conduct the extensive experiments against six state-of-the-art approaches on the existing dataset and from the real deployment environment. The experimental results confirm that our approach can significantly outperform current state-of-the-art baselines.

==> bio.tex <==
\vspace{10cm}

\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{avatar/wubozhi.jpg}}]
{Bozhi Wu} is currently pursuing the Ph.D. degree in computer science at Nanyang Technological University, Singapore. His research interests include malware detection, vulnerability detection and deep learning. He focuses on solving conventional problems in software engineering with AI technology.
\end{IEEEbiography}

\vspace{-1.5cm}

\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{avatar/sql.jpeg}}]
{Shangqing Liu} is a research associate at Nanyang Technological University, Singapore. His Ph.D study is supervised by Prof. Liu Yang from NTU. Previously, he was an intern student at Nanyang Technological University from 2017 to 2018. His research interests include graph neural networks (GNNs), program representation learning.
\end{IEEEbiography}

\vspace{-1.5cm}

\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{avatar/rtfeng.png}}]
{Ruitao Feng} received his B.S. degree from the Tianjin University in 2014 and his Ph.D. degree from the Nanyang Technological University in 2021. He is now a research fellow in Nanyang Technological University since 2021. Previously, he was a research assistant in Nanyang Technological University from 2014 to 2020.
His research interests include discovering and solving security problems on mobile platform, IoT system and AI-based cybersecurity system.
\end{IEEEbiography}

\vspace{-1.5cm}

\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{avatar/fei.jpeg}}]
{Xiaofei Xie} received his Ph.D, M.E. and B.E. from Tianjin University. He is currently an assistant professor in Singapore Management University, Singapore. His research mainly focuses on program analysis, traditional software testing and quality assurance analysis of deep learning systems.
He has published some top tier conference/journal papers relevant to software analysis and won two ACM SIGSOFT Distinguished Paper Awards. 
% in FSE'16 and ASE’19
% in ICSE, ISSTA, FSE, ASE, TDSC, TIFS, TSE, IJCAI, NeurIPS, ICML and CCS. In particular, he won two ACM SIGSOFT Distinguished Paper Awards in FSE'16 and ASE’19.
\end{IEEEbiography}

\vspace{-1.5cm}

\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{avatar/jingkai.jpg}}]
{Jingkai Siow} is currently pursuing his Ph.D. in computer science at Nanyang Technological University, and holds a B.A. in computer science from the Nanyang Technological University. He is also a research graduate officer at Nanyang Technological University. His area of research involves deep learning, cyber-security, and software engineering.
He has more than four years of research experience, software development and data engineering.
% , and is proficient in software and data engineering. 
\end{IEEEbiography}

\vspace{-1.5cm}

\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{avatar/shangwei.jpg}}]
{Shangwei Lin} received his B.S. and Ph.D. degree from the National Chung Cheng University in 2003 and 2010. He worked as post-doctoral researcher at NUS and SUTD from 2011 to 2015. In May 2015, he joined NTU as Assistant Professor. His research interests include formal verification, formal synthesis, embedded system design, cyberphysical systems, security systems, multi-core programming, and component-based object-oriented app frameworks for real-time embedded systems. 
\end{IEEEbiography}

% \vspace{-1.5cm}
\vspace{8cm}
